"President Vows to Cut <Taxes> Hair": Dataset and Analysis of Creative Text Editing for Humorous Headlines

We introduce, release, and analyze a new dataset, called Humicroedit, for research in computational humor. Our publicly available data consists of regular English news headlines paired with versions of the same headlines that contain simple replacement edits designed to make them funny. We carefully curated crowdsourced editors to create funny headlines and judges to score a to a total of 15,095 edited headlines, with five judges per headline. The simple edits, usually just a single word replacement, mean we can apply straightforward analysis techniques to determine what makes our edited headlines humorous. We show how the data support classic theories of humor, such as incongruity, superiority, and setup/punchline. Finally, we develop baseline classifiers that can predict whether or not an edited headline is funny, which is a first step toward automatically generating humorous headlines as an approach to creating topical humor.

==> headline-humor.tex <==
Computational humor research, particularly humor generation, is still in its nascent stages. Part of the problem is the lack of training datasets for generating humor. In this paper, we introduce a new benchmark for humor research by building a dataset of news headlines, applying crowd-sourcing to edit them to make them funny and to assess the funniness of these edits, and creating a gold standard of 15,000 headline edits annotated for funniness.
%we apply crowd-sourcing to edit these headlines to make them funny and to assess the funniness of the edits, obtaining a total of 15,000 news headline edits annotated for funniness.
Next, we perform various analyses on the dataset to study what makes an edited headline humorous. We then develop several algorithms to predict whether an edited headline is funny. Our results demonstrate various agreements with classic humor theories, and we make our dataset public to facilitate research on computerized humor recognition and generation.


\section{Introduction}
Computational humor continues to be quite a challenging problem. While there have been some advancements on automatic humor recognition~\addcite{}, computerized humor generation has seen very little progress. Humor understanding requires reasoning at multiple levels of cognition, in-depth world-knowledge, common sense, and the ability to comprehend connections between entities at various levels of cognition, making research on this area notoriously difficult.

%Importantly enough, 
A big hindrance to progress on humor research is the lack of public datasets. Furthermore, the few datasets out there address specific sub-tasks for humor such as detecting funny one-liners\addcite{}, puns\addcite{}, \etc{} Creating a humor dataset is non-trivial because it requires (i) human annotators which makes the process expensive and time-consuming, and (ii) a clear definition of humor so that annotators have good agreements among each other.

In this paper, we introduce a novel benchmark to facilitate research on computational humor. We collect original news headlines from various news media posted on Reddit\footnote{\texttt{www.reddit.com}}. Then, we {\it qualify} expert annotators from Amazon Mechanical Turk\footnote{\texttt{www.mturk.com}} to generate humor by editing these headlines and to judge the humor in these edits. Our resulting dataset called \textcolor{red}{XXX}, containing 15,000 edited news headlines and their humor assessed, enables various humor tasks, such as to:
\begin{enumerate}
    \item Predict whether an edited headline is funny.
    \item Rank multiple edits of the same headline on a funniness scale.
    \item Generate humorous news headlines.
    \item Recommend funny headlines personalized to a reader.
\end{enumerate}
A screenshot of our annotation tasks is shown in Figure~\ref{fig:mturkScreenShots}, and sample edited headlines from our dataset are shown in  Table~\ref{tab:headline_edits}. 

Our benchmark shall help the community focus on interesting challenges in humor research since: 
%\mg{should use different language here, we should stress that we help humor research, maybe "allow humor research to focus on some interesting challenges such as:"} %poses various challenges to humor research because:
\begin{enumerate}
    \item Headlines have very little context, but convey a lot of information.
    \item A thorough understanding of world-knowledge and common-sense is needed to understand what makes a headline funny.
    \item Humorous headlines are often generated using several \textcolor{red}{layers} %levels
    of cognition and reasoning.
    \item Despite us carefully qualifying annotators, their knowledge, preferences, bias and stance towards %entities and issues mentioned 
    information presented in headlines influence whether they perceive a potentially funny headline as humorous, offensive, confusing, \etc{}
\end{enumerate}
The presence of these factors means humor understanding in our dataset requires the development of NLP tools that are not only robust at pattern recognition but also capable of reasoning and perception --- areas where progress has been notoriously difficult.
%challenge NLP tools Our expectation is that \mg{redundant - don't mention "serious challenges" here} these factors will make humor understanding require NLP tools demand for development of NLP tools for perception and reasoning pose serious challenges to current NLP tools and help improve the state-of-the-art in humor research.

% TODO: Describe analysis, results, classification

We will now describe the task and the data collection steps.
\begin{figure}
    \centering
    \begin{tabular}{c}
      \resizebox{0.95\columnwidth}{!}{\fbox{
        \includegraphics{figures/mturkEdit.png}}} \\ (a) The  Editing Task. \\ \\
      \resizebox{0.95\columnwidth}{!}{\fbox{
        \includegraphics{figures/mturkGrade.png}}} \\ (b) The Grading Task. \\
    \end{tabular}
  \caption{Screenshots of the headline editing and grading interfaces. Only the underlined tokens are replaceable.}
  \label{fig:mturkScreenShots}
\end{figure}

%Table~\ref{tab:headline_edits} shows sample headline edits from our dataset, capturing different funniness approaches.
 \begin{table*}
     \centering
     \resizebox{\textwidth}{!}{        
    \begin{tabular}{|l|l|}
        \hline
         {\bf Headline} & {\bf Substitute} \\ \hline
           Trump cancels meeting with {\bf \textcolor{red}{North Korea}}, citing `tremendous anger and open hostility' & \textcolor{darkGreen}{wife} \\ \hline
          101 {\bf \textcolor{red}{Illegal Immigrants}} Arrested in ICE Operation, a Christmas Gift from ICE & \textcolor{darkGreen}{dalmations} \\ \hline
           UK set to ban {\bf \textcolor{red}{laptops}} on flights from Middle East countries & \textcolor{darkGreen}{pillows} \\ \hline
           Kushner to visit {\bf \textcolor{red}{Mexico}} following latest Trump tirades & \textcolor{darkGreen}{therapist} \\ \hline 
          Mac users, you need to change your {\bf \textcolor{red}{passwords}} immediately!!  & \textcolor{darkGreen}{underwear} \\ \hline
          Trump wants you to take his {\bf \textcolor{red}{tweets}} seriously. His aides don't & \textcolor{darkGreen}{hair} \\ \hline
          Essential Politics: California's hottest congressional {\bf \textcolor{red}{races}}, ranked & \textcolor{darkGreen}{mistresses} \\ \hline
          %{\bf \textcolor{red}{Facts}} Have a Well-Known Liberal Bias & \textcolor{darkGreen}{Liberals}\\ \hline
         
          
     \end{tabular}}
     \caption{Some headlines in our dataset and their edits.}
     \label{tab:headline_edits}
 \end{table*}
 
 
 
 
 
 
 
 \iffalse
     \begin{tabular}{|L{8cm}|C{1.7cm}|}
         Headline & Substitute \\ \hline
          Kushner to visit {\bf \textcolor{red}{Mexico}} following latest Trump tirades & \textcolor{darkGreen}{therapist} \\ \hline 
          Mac users, you need to change your {\bf \textcolor{red}{passwords}} immediately!!  & \textcolor{darkGreen}{underwear} \\ \hline
          Trump wants you to take his {\bf \textcolor{red}{tweets}} seriously. His aides don't & \textcolor{darkGreen}{hair} \\ \hline
          Essential Politics: California's hottest congressional {\bf \textcolor{red}{races}}, ranked & \textcolor{darkGreen}{mistresses} \\ \hline
          
               \begin{tabular}{|l|}
          \hline
          Kushner to visit {\bf \textcolor{red}{Mexico}}/\textcolor{darkGreen}{therapist} following latest Trump tirades  \\ \hline 
          Mac users, you need to change your {\bf \textcolor{red}{passwords}}/\textcolor{darkGreen}{underwear} immediately!!  \\ \hline
          Trump wants you to take his {\bf \textcolor{red}{tweets}}/\textcolor{darkGreen}{hair} seriously. His aides don't  \\ \hline
          Essential Politics: California's hottest congressional {\bf \textcolor{red}{races}}/\textcolor{darkGreen}{mistresses}, ranked \\ \hline
\fi \section{The Humor Dataset}

We gathered thousands of original headlines, directed editors to make them funny, and employed graders to assess their level of humor.

\iffalse
JOHN To Do: describe bing news data collection; mention start and end dates

\subsection{News Headline Data}

Politics and Science/Technology

random sampling --- at least 1 entity (from 90+ percentile) --- Max TFIDF difference === 10000 headlines
\fi

% TODO: annotation problem: knowledge, mode, exhaustion, no more surprise with passage of time
\subsection{Task Description}
%NOTE: Describe motivation behind task design, 1 word substitution rule decision, etc.
Our goal is to study how humor can be generated by applying edits to short chunks of text, such as phrases or sentences, which have very little context. 
%obtain a dataset of small edits applied to \mg{should we say "short strings" instead of "sentences" otherwise the reader might get confused to why we suddenly switch from "headlines" to "sentences" in the discussion?} sentences to make them humorous. 
However, not all such text can be made funny, particularly because, standalone, they usually do not convey enough information. To this end, news headlines are useful because of the rich information content they present despite their sentence-like short form. Moreover, our additional goal is to generate humor given severe restrictions on editing flexibility so that the edit does not significantly change the headline context and the majority of the information conveyed.

Therefore, our task is to {\bf humorify} a headline, \ie{} {\it edit} a headline to make it funny, where an {\bf edit} %NOTE: call it HEdit? = Headline + Edit
is defined as a substitution of a single-word verb or noun, or an entity, with a single-word that is a verb or a noun\footnote{During pilot tests, we allowed multi-word addition and/or deletion, but we found that annotators were then making very noisy edits which would make the resulting dataset too complex.}. That is, an editor was allowed to insert a single-word verb or noun to replace an existing entity or single-word verb or noun. %while preserving subject-verb agreement. 
% NOTE: substitute "edit" with a more catchy term that we can keep referring later and people wont be confused as to what edit we allow? e.g. morph/h-edit/funEdit?
Note that we do not allow:
\begin{itemize}
    \item Addition/removal of a whole noun/verb phrase, except removal of noun phrases that are entities (\eg{} One World, Virtual Reality).
    \item Removal of sub-tokens within entities (\ie{} replacing only the word ``States'' in ``United States'').
\end{itemize}
%Some entities can be noun phrases (\eg{} Virtual Reality), and in these cases, we rely on the intelligence of the editors to remove tokens that are dominantly entities as opposed to noun phrases. Our expectation is that our funny headline generator will be able to learn from signals in the editors' chosen replaced words to prevent itself from replacing exclusive noun phrases.
%NOTE: Describe why not adjectives, adverbs, etc. other POS. 
The decision to strictly avoid edits of other parts-of-speech (POS) words was motivated by the textcolor{re}{fact/observation} that they did not provide enough variety of humor. For example, when substituting adjectives and adverbs for humor, people mostly use antonyms or superlatives (\addcite--- MadLibs paper?).
%attempt humor generation using antonyms or superlatives, which are one-dimensional, and not interesting. 
Contrarily, switching nouns and verbs allows room for making diverse connections between entities and actions mentioned in the headline.

To obtain the replaceable words in each headline, first we apply named entity recognition (NER) and POS tagging using the Stanford CoreNLP toolkit~\cite{manning-corenlp} to find the entities, nouns and verbs. We allow for replacement of only those entities that are well-known according to the Microsoft Knowledge Base\addcite. This raises the chances that annotators are familiar with the replaceable entity which helps to edit it for funniness and to judge the humor generated by the edit. %and not frequent according to the Google N-gram corpus\footnote{https://catalog.ldc.upenn.edu/LDC2006T13}
Then, we allow a noun (or verb) to be replaced if it\footnote{its singular form in the case of a plural noun} is a strict noun (or verb) in WordNet~\cite{fellbaum1998wordnet} (\ie{} does not have a WordNet entry with another POS).

\iffalse
We make use of the following two word lists for our experiments:
\begin{itemize}
    \item NList: a list of words in WordNet~\cite{fellbaum1998wordnet} that have a noun entry but do not have a verb, adjective or adverb entry. This list has 62,679 tokens.
    \item EList: a list of entities obtained from Microsoft Knowledge Base\addcite. This list was further filtered by removing frequent tokens according to the Google N-gram corpus\footnote{https://catalog.ldc.upenn.edu/LDC2006T13}.
\end{itemize}

We apply the following rules to select candidate tokens from the headline to replace. Selected tokens must be one of the following:
\begin{enumerate}
    \item a single-word noun according to the Stanford Caseless Part of Speech Tagger\footnote{https://stanfordnlp.github.io/CoreNLP/caseless.html} which can be found in NList. %If the token is a plural noun, we check if its singular format is in NList.
    \item an entity in EList.
    %\item a single word not found in WordNet. We believe these could be out of vocabulary nouns (\eg{} ``app'').
\end{enumerate}
When we identify entity tokens in a headline, we remove the tokens that are subsets of other entities found in the same headline (e.g. we only keep ``The United States of America'' and exclude ``United States'' and ``America'').

When our algorithm generates possible substitute candidates for a token, we only take those candidates which belong to NList or EList. Therefore, we have a finite set of substitute words.
\fi



\subsection{Collecting Headlines}
%TODO: Emphasizing why using popular headlines is so important for getting better humor. i.e. audience needs to understand the entities, event, information mentioned in the headline in order to understand how humorous an edit is, also humor generator (turker/machine) needs to know about the entities, event, information in order to edit the headline into a funny headline.

We build our news headlines dataset from the social media site Reddit. The advantage of using Reddit is that the vast majority of news headlines posted there are frequently shared amongst a general audience. This steers us towards a set of headlines that is more likely to be part of general discourse, rather than specialized content that might not be common knowledge to the general population which would make editing them for humor difficult.
%desirable than obtaining headlines directly from news sources' websites which contain many headlines that include events and entities not known to people which would make editing them for humor difficult.

We obtain all Reddit posts from the subreddits \texttt{/r/worldnews} and \texttt{/r/politics} %NOTE: we can justify why we selected world news and politics using Pew research data which found that these are 2 of the top 3 news categories people are mostly interested about
from January 2017 to May 2018 using Google BigQuery\footnote{\texttt{https://cloud.google.com/bigquery}}. Each of these posts is a headline from a news source. 
%, and we get 2,206,392 headlines from XXX unique news sources. 
Then, we remove all headlines that have less than 4 words or more than 20 words. Next, we resolve duplicate headlines arising from multiple sources by keeping only the headline and the source for which the Reddit post had the highest number of Reddit user comments followed by the earliest publication timestamp\footnote{we also resolved duplicates by merging multiple sites of the same news source, \eg{} \{www, edition, money\}.cnn.com.}. 
%Then, we count the number of headlines per news source and keep only the headlines from the top 25 news sources according to this number.  These steps help us keep the popular news sources, and we get a total of 287,076 headlines\footnote{Dataset link will be provided upon publication.}.
Then, we keep all the headlines from the top 25 most-frequent news sources based on number of their headlines, and we obtain a total of 287,076 headlines.

\subsection{Annotation}
%Our goal is to obtain a labeled dataset with high funniness grades. Therefore, we apply an iterative data annotation approach. We will have $N$ rounds of data annotation, where after completion of each $n$-th round ($1\leq n<N$), we will train a classifier to give us headlines that have higher potential to be funny (\ie{} they can be more easily made humorous with an edit), and we will apply this classifier to sample data for the $(n+1)$-th round.

%We crowd source our data annotation task using Amazon Mechanical Turk. 
For our data annotation task, we use mechanical turk workers who (i) are located in the U.S., (ii) have a HIT approval rate greater than $97\%$, and (iii) have more than 10,000 HITs approved.
Moreover, since generating and recognizing humor are challenging
% NOTE: should I say non-trivial/quite difficult?
tasks, we further qualify distinct sets of turker (i) judges specialized at recognizing humor in an edited headline, and (ii) editors adept at editing headlines to generate humor. %\mg{the two separate tasks need to be called out more explicitly, maybe as bullets, otherwise readers might get lost in the following subsections. Title of next subsection should be "Qualifying Humor Judges" and 2.3.2 should be "Qualifying Humor Editors"}

\subsubsection{Qualifying Humor Judges}
We manually collected a set of 20 original news headlines and edited each of them carefully such that some edits are funny and some are not. We asked %10 
several internal judges in our research group to judge the funniness of each edited headline using the following integer scale:
\vspace{2pt}
\begin{center}
\begin{tabular}{lcl}
{\bf 0} - Not funny   &  &  {\bf 1} - Somewhat funny \\
{\bf 2} - Moderately funny &   & {\bf 3} - Funny
\end{tabular}
\end{center}
\vspace{2pt}
We instructed judges to grade objectively:
\begin{itemize}
    \item regardless of their own stance towards issues, entities and information expressed in the headline, and to
    \item grade the headline as funny if they believed it would be funny to a large audience.
\end{itemize}.
Finally, we instructed judges to grade an edited headline funny if either:
\begin{itemize}
    \item the headline was funny by itself regardless of the original headline, or
    \item the headline was only funny when considering how the original headline was changed.
\end{itemize}
We labeled the ground truth funniness score of each headline as its mean internal judge grade. Table~\ref{tab:gtruth_internal_judges} describes these ground truth grades.
\begin{table}
    \centering
    \begin{tabular}{c|c|c}
         Grade Range & Class Label & \# Headlines \\ \hline
         0.0 - 0.6 & Not Funny & 10 \\
         1.0 - 1.9 & Funny & 7 \\ 
         2.0 - 2.4 & Funny & 3 \\
    \end{tabular}
    \caption{Internal judges' mean funniness grades for headlines.}
    \label{tab:gtruth_internal_judges}
\end{table}

%Next, we used 150 turkers to do the same task.
We launched the same task on Mechanical Turk until we found 150 qualified judges. Turkers were qualified if:
\begin{itemize}
    \item they had 3 or less {\it Class Label} errors according to Table~\ref{tab:gtruth_internal_judges}, and
    \item on average, their grades were within $0.6$ of the mean internal judge grades.

\end{itemize} 

We calculated inter-annotator agreements for assigning headline funniness grades using Krippendorf's Alpha~\cite{krippendorff1970estimating} interval metric --- a real number in the interval [-1,1], with -1, 0 and 1, respectively, implying complete disagreement, no consensus and full agreement. 
%We calculated the inter-annotator agreement among our internal judges using Krippendorf's Alpha~\cite{krippendorff1970estimating}. 
%Alpha is a real number in the interval $[-1,1]$, with $-1$, $0$ and $1$ implying, respectively, complete disagreement, no consensus, and full agreement. 
The alpha for the internal judges and qualified turkers were, respectively, $0.569$ and $0.636$. %\mg{the next statement is a bit iffy because there is no agreement in the literature as to what exactly counts as "good" agreement in Krippendorf metrics. I'd just mention the numbers and leave it at that.} both implying strong agreement. 
%NOTE: need to re-calculate judges' agreement now that we have a bigger judge pool

\subsubsection{Qualifying Humor Editors}
We launched 6 editor qualification tasks, each with 10 original headlines that turkers were asked to make as funny as possible to a general audience. We carefully chose headlines for each task to the best of our judgment such that the tasks were ``easy'', ``medium'', or ``hard'' in terms of making their headlines funny by editing. 

We instructed task participants not to perform the following edits which we consider as {\bf rule violations}:
\begin{itemize}
    \item Cheap humor generation techniques: add profanity, slang, bathroom/potty humor, sexual reference or informal language.
    \item Squeeze multiple words into one (\eg{} Housecat, JumpedOverWall).
\end{itemize}

For each task, we used 30-35 turkers, and then we graded the funniness of each edited headline using 7 of our qualified judges. Next, we calculated the average funniness grade of a story per task, which were 0.91, 0.95 and 1.07 respectively. Finally, we calculated the average funniness grade of each task participant and selected him/her as a qualified editor if the average funniness grade of his edits was above $0.8$ or the task's average story's funniness grade, whichever was higher. In total, we obtained 100 qualified editors.

\subsection{Data Collection and Quality Control}
We randomly sampled a total of 5,000 news headlines from our Reddit dataset, obtaining roughly an equal number of headlines from each news source. Then, we asked 3 editors to edit each headline and 5 judges to grade each edited headline --- 
%and to mark the rule violations. 
this helps compare different edits of the same headline for funniness and to study what makes a certain edit funnier than another.

We implemented several methods to ensure quality control during data collection: %which we encourage future data collectors to apply.
\begin{itemize}
    \item To avoid turker exhaustion and decision fatigue, we performed the annotation task over a series of mini-batches launched at least 24 hours apart.
    \item After each round of editing, we applied tools to (i) check the edits for spelling mistakes which we manually corrected, and (ii) to find if an inserted token was actually two or more words squeezed into one (\eg{} pocketwatch, selftanner) which we discarded from the dataset before continuing to funniness grading.
    \item To allow diversity in annotations, we applied a maximum HIT limit for annotators per batch. After each batch, we temporarily suspended those editors and judges who had done significantly more HITs than the rest until the others caught up. 
\end{itemize}
Lastly, as we obtained more and more annotated data, the editors kept employing the same humor generation strategies (\eg{} inserting words from a small vocabulary, using similar words, \etc{}). Consequently, judges kept getting quite familiar with new edits having seen a lot of similar edits before, so the element of surprise was gone and the judges were grading fewer humorous edits as funny.
%not grading many humorous edits as funny because they had seen similar edits before. 
%We saw that the average funniness grade of an edit for the $n$-th batch was usually lower than the $(n-1)$-th batch.
We addressed these by randomly sampling a set of editors and judges for each batch, obtaining new editors and judges over time, and removing those editors who had done a majority of the HITs but their edits' average funniness grade fell below a threshold (=$0.7$) after they participated in a batch. %\mg{Isn't the next sentence just a rewording of the previous statements?} 
Moreover, we removed ``grumpy'' judges who developed an increasingly higher threshold for humor recognition over time by looking for judges who repeatedly assigned very low funniness grades compared to the 4 other judges for the same edit.

The minimum judge agreement score among all of our batches was %0.238 NOTE: need to re-calculate it
$0.146$ and the full dataset's agreement score was $0.178$, both showing reasonable consensus considering the factors above and other factors such as turkers' personal preferences, bias, political stance, \etc{} which make agreement difficult. %NOTE: need to update the minimum agreement and compute X at end of full data collection step.

Our full dataset includes a total of 15,000 annotated headlines\footnote{Annotated dataset will be shared upon publication.}. For annotating a single headline, we paid $10$ US cents to editors and $2.5$ US cents judges, and factoring in the costs for qualification, 
%\mg{do we need to mentionm total cost? --- Nabil: Yes, because that is what EMNLP reviewers asked us last time. Can put this in Appendix} 
our total cost for obtaining the dataset is about USD $4500$. We share our Mechanical Turk task instruction snapshots for headline editing and grading in the Appendix.




\section{Humor Analysis}
In this section, we analyze what types of edits create humor in our dataset and we compare our findings with humor theories.

\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{
        \includegraphics{figures/fun_potential.png}}
    \caption{Histogram of humor potentials of headlines.}
    \label{fig:headline_funniness_potential}
\end{figure}
Figure~\ref{fig:headline_funniness_potential} shows the histogram of {\bf headline funniness potential}, which we define per headline as the average of all the funniness grades (usually 15) received for all edits of each headline. The figure suggests that some headlines are inherently difficult to make humorous by editing, while the majority of headlines can be edited to achieve slight to moderate levels of humor.
%Note: can define and consistently use "humorify" = edit a headline to make it humorous

\begin{figure}
    \centering
    \resizebox{\columnwidth}{!}{
        \includegraphics{figures/mean_fun_grade.png}}
    \caption{Headline edit mean funniness histogram.}
    \label{fig:headline_avg_funniness}
\end{figure}
Figure~\ref{fig:headline_avg_funniness} shows the histogram of mean funniness grades for headline edits. 

%NOTE: Need discussion as to why the shape of the two histograms are different. Any conclusive relations between headline humor potential and headline edit funniness?

Table~\ref{tab:factors} presents insights into several features that may be factors that may be influential for humor generation. We investigated these factors in detail, and found the following results:
\begin{itemize}
    \item Number of words: Figure~\ref{fig:headline_vs_words} shows that the population of our collected headlines from Reddit has a length distribution similar to a normal distribution centered on a word count of 10. Interestingly, the highest and lowest funny headlines are generated towards the two extremes. This makes sense since very short headlines (4-5 words long) barely have enough contextual information to exploit to make a humorous edit whereas headlines that have very rich contexts  generally allow editors various types of edits to be made to generate humor.
    \item Number of replaceable words: In the dataset, this number ranged between 1 to 12, and funniness grades of edits were significantly low at the two extremes, in other words, editors had difficulty generating humor when they were severely constrained in choosing a word to replace, or when they had a huge number of choices for replacement.
    \item Proportion of replaceable words (see Figure~\ref{fig:funny_vs_proportion}): The higher the proportion of words that were replaceable, the higher the mean funniness was in general. This suggests that allowing editors more freedom in choosing words from the headline to edit results in better humor, or perhaps the higher the proportion of nouns, entities and verbs in the headline, the greater is the chance of humor generation.
\end{itemize}


\begin{table*}
    \centering
    \begin{tabular}{l||c|c|c|c|c|c}
        Factor & Mean & St.Dev & Min & Max & Corr. & Relation \\ \hline
        Number of words & & & & & & \\ \hline
        Number of replaceable words & & & & & & \\ \hline
        Proportion of word that are replaceable & & & & & & \\ \hline
    \end{tabular}
    \caption{Summary of different factors that may play a part in humor generation, and their correlation with the edit's funniness grade.}
    \label{tab:factors}
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/numWords_plots.png}
    \caption{Impact of number of words in headline towards humorous headline edit generation.}
    \label{fig:headline_vs_words}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/funniness_vs_replaceables_proportion_5.png}
    \caption{Higher proportion of words that are replaceable leads to higher funniness of edits.}
    \label{fig:funny_vs_proportion}
\end{figure}
    
\subsection{Qualitative Analysis of Joke Generation Strategies}
NOTE: Discuss humor generation strategies editors have applied, give evidence from Table 1. Mention that we have political humor, which makes the task difficult for agreement.


\subsection{Joke Profile}
\mg{this headline is confusing since we have not introduced any notion of "joke"}

%5.	Joke profile for editing (the histogram count of the relative position of words that were replaced. Relative position = word position / number of words in headline).

We specifically study whether the ``setup and punchline''\addcite approach is used in funny headline generation. For this, we construct the {\bf joke profile graph}, shown in Figure~\ref{fig:joke_profile}. It shows the proportion of time the editors substituted a word at each relative word position bin (a measure of the ``tendency'' of editors to remove a word from each relative position)  compared to if they randomly chose a word to substitute. 

Clearly, the editors are substituting fewer words from the early parts of headlines compared to random substitution, and they are substituting much more words from the latter parts of the headline than random choice warrants, suggesting that editors are attempting the ``setup and punchline'' approach for humor generation. Furthermore, the difference between the actual substitution and random substitution at each relative position is monotonically increasing.

Furthermore, Figure~\ref{fig:joke_profile} shows that substitutions further along in the headline receive higher funniness grades which suggests that the ``setup and punchline'' approach is helping to amuse the judges.

%Clearly, editors are intentionally choosing to substitute less from the early part of the headline and more from the latter part, much less than they would if they randomly picked words to replace, plus they are intentionally choosing to replace words from the latter part of the headline much more than they would if they randomly picked words to replace — this suggests that they are attempting the setup and punchline approach. Also note that the blue line for the 5 bin case is monotonically increasing.

%The red line shows the probability of a random word replacement, the green line shows the proportion of time the turkers chose to remove a word from each relative position bin, and the blue line = green line - red line. Interpretation: Turkers are intentionally choosing to replace words from the early part of the headline much less than they would if they randomly picked words to replace, plus they are intentionally choosing to replace words from the latter part of the headline much more than they would if they randomly picked words to replace — this suggests that they are attempting the setup and punchline approach. Also note that the blue line for the 5 bin case is monotonically increasing.
%6.	Joke profile after grading (same as joke profile for editing, but the counts were weighed by the funniness grades). We plot for bin widths of 0.1 and 0.2.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/joke_profile_graph_numBins_10.png}
    \caption{The joke profile graph.}
    \label{fig:joke_profile}
\end{figure}

%\subsection{Feature Correlations}
%NOTE: Discuss feature correlations



\section{Detecting Funny Headlines}

\subsection{Features}

\subsection{Classification}

\subsection{Results}

\iffalse
\subsection{High Potential Headline Generator}
\subsection{Iterative Data Annotation}
\section{Funny Headline Generator}
\subsection{Features}
\subsection{Classification}
\fi


